Cognitive network science reveals bias in GPT-3, ChatGPT, and GPT-4 mirroring math anxiety in high-school students

Large language models are becoming increasingly integrated into our lives. Hence, it is important to understand the biases present in their outputs in order to avoid perpetuating harmful stereotypes, which originate in our own flawed ways of thinking. This challenge requires developing new benchmarks and methods for quantifying affective and semantic bias, keeping in mind that LLMs act as psycho-social mirrors that reflect the views and tendencies that are prevalent in society. One such tendency that has harmful negative effects is the global phenomenon of anxiety toward math and STEM subjects. Here, we investigate perceptions of math and STEM fields provided by cutting-edge language models, namely GPT-3, Chat-GPT, and GPT-4, by applying an approach from network science and cognitive psychology. Specifically, we use behavioral forma mentis networks (BFMNs) to understand how these LLMs frame math and STEM disciplines in relation to other concepts. We use data obtained by probing the three LLMs in a language generation task that has previously been applied to humans. Our findings indicate that LLMs have an overall negative perception of math and STEM fields, with math being perceived most negatively. We observe significant differences across the three LLMs. We observe that newer versions (i.e. GPT-4) produce richer, more complex perceptions as well as less negative perceptions compared to older versions and N=159 high-school students. These findings suggest that advances in the architecture of LLMs may lead to increasingly less biased models that could even perhaps someday aid in reducing harmful stereotypes in society rather than perpetuating them.

==> bozzatemp.tex <==
[Hagendorff]

Due to rapid technological advances and their extreme
versatility, LLMs nowadays have millions of users and are at the cusp of being the main go-to technology
for information retrieval, content generation, problem-solving, etc. Therefore, it is of great importance to
thoroughly assess and scrutinize their capabilities. Due to increasingly complex and novel behavioral
patterns in current LLMs, this can be done by treating them as participants in psychology experiments
that were originally designed to test humans. For this purpose, the paper introduces a new field of research
called “machine psychology”.

In sum, machine psychology aims to discover emergent abilities in LLMs
that cannot be detected by most traditional natural language processing benchmarks.

Moreover, LLMs are at the cusp of being deployed as search engines and virtual assistants in
high-stakes areas, thus impacting societies at large. In other words, next to humans, LLMs are increasingly
becoming important contributors to the infosphere, causing immense societal changes by normalizing
communicative relations between humans and artificial systems.

However, due to the ability of LLMs to reason and to engage in opendomain conversations, new and further-reaching opportunities for investigating traits and behavioral
patterns of LLMs become necessary.

This is where machine psychology comes into play. It aims to elicit mechanisms of decision-making and
reasoning in LLMs by treating them as participants in psychology experiments. Decades of researching
humans and “accessing” the human psyche via language-based tools resulted in a plethora of methods
and test frameworks that can now be harnessed to investigate not just humans, but also artificial agents.
Since the increase in capabilities in artificial neural nets, especially transformers (Vaswani et al. 2017),
has led to an increase in technical opacity, too, it is promising to borrow these methods that were designed
to investigate another opaque structure, namely biological neural nets.

However, while traditional benchmarking primarily aims at optimizing LLMs against the
backdrop of specific metrics, machine psychology is not primarily interested in increasing an LLM’s performance. In addition to that, compared to traditional natural language processing benchmarks that
measure abilities such as reading comprehension, translation, numerical reasoning, paraphrasing,
truthfulness, etc., machine psychology can tackle broader, more complex scenarios and identify high-level
traits in individual LLMs as well as in multiple instances of an LLM interacting with each other by using
prompt chains (Wu et al. 2022). This is, among others, especially important for AI safety and alignment
research (Amodei et al. 2017; Hendrycks et al. 2022; Hendrycks and Mazeika 2022), which tries to identify
emergent properties such as goal setting, self-awareness, deceptiveness, or other potentially malevolent
and unsafe behavior in AI systems that are indiscernible in a low-level analysis as well as largely
overlooked in entrenched auditing frameworks (Mökander et al. 2023).

However, when sticking to purely language-based approaches, among
the many methodical approaches used in human psychology, at least two approaches can be directly
transferred to machine psychology. First, self-report methods such as interviews and questionnaires can
(if enough scaling is provided) elicit systematic information about LLMs by measuring the prevalence of
certain attitudes or behaviors.

LLMs use prompts to guide their learning and decision-making processes; and the quality of these prompts
determines the accuracy, quality, and effectiveness of the system’s responses. However, LLMs are very
sensitive to prompt wording, meaning that even slight changes in the wording can result in significant
differences in prompt completions. This makes machine psychology studies prone to p-hacking [QUESTO E' RILEVANTE PER DISCUTERE LE PERCENTUALI DI ERRORI SU PROMPT IDENTICI]

FONDAMENTALE TABELLA 2
1. Avoid training data contamination: They use prompts from psychology studies and apply them to LLMs without changing their wording, task orders, etc. This way, LLMs are likely to have already experienced identical or very similar tasks during training, thus causing LLMs to just reproduce known token patterns. When adopting test frameworks from psychology – meaning vignettes, questionnaires, or other test setups – one must ensure that the LLM has never seen the tests before and go beyond mere memorization.
2. Multiply prompts: Because of this high sensitivity to prompt wording, it is
important to test multiple versions of one task and to create representative samples, meaning batteries
of slightly varied prompts. Only this way can one reliably measure whether a certain behavior is
systematically reoccurring and generalizable.

LLMs are, like the human brain, black boxes. By applying psychological terms to them,
the explanatory power increases, even though no direct artificial neural correlates to these terms exist. [USARE PER CHIUDERE LA DISCUSSIONE INVERTENDO IL SIGNIFICATO DELLA FRASE: magari è vero che sono entrambe delle black boxes, ma non tutte le black boxes sono al loro interno uguali!]

[SECONDO PAPER SULL'IMPORTANZA DEI BIAS NEI LLMS]
This paper stresses the importance of biases in the field of artificial intelligence (AI). To foster efficient algorithmic decision-making in complex, unstable, and uncertain real-world environments, we argue for the implementation of human cognitive biases in learning algorithms. We use insights from cognitive science and apply them to the AI field, combining theoretical considerations with tangible examples depicting promising bias implementation scenarios. Ultimately, this paper is the first tentative step to explicitly putting the idea forth to implement cognitive biases into machines.





[Griffiths]
Recent progress in artificial intelligence provides the opportunity to ask the
question of what is unique about human intelligence, but with a new comparison
class. I argue that we can understand human intelligence, and the ways in which
it may differ from artificial intelligence, by considering the characteristics of the
kind of computational problems that human minds have to solve. I claim that
these problems acquire their structure from three fundamental limitations that
apply to human beings: limited time, limited computation, and limited
communication. From these limitations we can derive many of the properties
we associate with human intelligence, such as rapid learning, the ability to
break down problems into parts, and the capacity for cumulative cultural
evolution.


